ToDER: Towards Colonoscopy Depth Estimation and Reconstruction with Geometry Constraint Adaptation

Visualizing colonoscopy is crucial for medical auxiliary diagnosis to prevent undetected polyps in areas that are not fully observed. Traditional feature-based and depth-based reconstruction approaches usually end up with undesirable results due to incorrect point matching or imprecise depth estimation in realistic colonoscopy videos. Modern deep-based methods often require a sufficient number of ground truth samples, which are generally hard to obtain in optical colonoscopy. To address this issue, self-supervised and domain adaptation methods have been explored. However, these methods neglect geometry constraints and exhibit lower accuracy in predicting detailed depth. We thus propose a novel reconstruction pipeline with a bi-directional adaptation architecture named ToDER to get precise depth estimations. Furthermore, we carefully design a TNet module in our adaptation architecture to yield geometry constraints and obtain better depth quality. Estimated depth is finally utilized to reconstruct a reliable colon model for visualization. Experimental results demonstrate that our approach can precisely predict depth maps in both realistic and synthetic colonoscopy videos compared with other self-supervised and domain adaptation methods. Our method on realistic colonoscopy also shows the great potential for visualizing unobserved regions and preventing misdiagnoses.

==> brief_sections/2_related_work_NOT_USING.tex <==
\section{Related work}

In this section, we will review 3D reconstruction and monocular depth estimation works in natural scenarios, especially the methods to obtain depth maps when the ground truth is not available, and their use for reconstruction in colonoscopy videos. 

% Reconstruction
\subsection{Colon reconstruction}
3D reconstruction has made impressive progress in various natural scenarios, such as indoor scenes and aerial view reconstruction. However, these methods perform poorly in the context of colonoscopy videos due to the poor quality of image features. Traditional reconstruction methods in colonoscopy often consider illumination-invariant descriptors~\cite{trink2017general} and optimize SLAM framework parameters~\cite{binhicip2019,Phan2020}. Zhang \textit{et al.}~\cite{zhang2020template} built a virtual colonoscopy environment based on a 3D colon model. Depth information also plays a crucial role in guiding 3D reconstruction and has been extensively explored in deep learning-based methods. For instance, RNN-SLAM~\cite{ma2021rnnslam} obtains depth and poses using a recurrent neural network, enabling real-time reconstruction. ColDe~\cite{zhang2021colde} designed a set of training losses to enhance depth and reconstruction results. $C^3$Fusion~\cite{posner2022c} utilizes contrastive deep features and consistent depth maps to improve upon the previous framework~\cite{zhang2021colde}. However, these reconstruction methods adopt a self-supervised approach, requiring more training data and higher training difficulty compared to domain adaptation methods.

\subsection{Depth Estimation}

Depth estimation takes images from a camera as input and measures the distance of each pixel from the shooting camera. This task is essential for visual perception but is an ill-posed problem. Traditional methods for depth estimation consider correspondence search, triangulation, and model fitting~\cite{geiger2011stereoscan,schonberger2016structure}. These methods compute depth using stereo images based on epipolar geometry, requiring at least two views. Recently, deep learning methods have come to dominate most visual understanding tasks, including depth estimation. Thanks to datasets with labeled depth information~\cite{geiger2012we,silberman2012indoor}, supervised depth estimation methods can predict depth using convolutional networks~\cite{liu2015learning,fu2018deep}, transformers~\cite{li2022binsformer}, or diffusion models~\cite{zhao2023unleashing}. Although these methods can achieve depth estimates close to actual distances, they rely on supervision from ground truth depth maps.

The acquisition of ground truth depth typically involves the use of depth cameras or manual labeling, adding to the cost and limiting potential application scenarios. To address cases where ground truth depth is unavailable, unsupervised and domain adaptation methods have been explored. In particular, inspired by~\cite{garg2016unsupervised}, various self-supervised monocular depth estimation methods have studied temporal consistency~\cite{zhan2018unsupervised}, adversarial learning~\cite{pilzer2018unsupervised}, and uncertainty~\cite{poggi2020uncertainty} to enhance the framework. However, their methods are built upon stereo consistency and require well-calibrated additional cameras. Domain adaptation methods focus on adapting depth models trained on one domain to other domains. S2R-DepthNet~\cite{chen2021s2r} learns a generalizable depth representation for natural scenes. However, applying these methods to colonoscopy videos is challenging due to the substantial domain gap between natural images and colonoscopy videos. Domain adaptation for synthetic colonoscopy imagery has also been explored. Mahmood \textit{et al.}\cite{mahmood2018unsupervised} transform realistic images into the synthetic domain to predict depth. Rau \textit{et al.}\cite{rau2019implicit} train a generative model on synthetic data, demonstrating implicit domain adaptation. These methods can be further enhanced to address challenges posed by inferior image features and complex noise.





==> brief_sections/figures/depth_real.tex <==
\begin{figure}[ht]
	\centering
	\includegraphics[width=0.7\textwidth]{figure/depth22.pdf}
 	% \vspace{-2mm}
	\caption{Depth estimation results for realistic colonoscopy. In comparison to other methods, \textit{ToDER} exhibits a higher capability for generating reasonable depths estimations, as indicated by the blue box. This observation underscores its ability to capture geometric details effectively.}
	\label{fig:depth_real}
 	% \vspace{-2mm}
\end{figure}

==> brief_sections/figures/depth_syn.tex <==
\begin{figure}[ht]
	\centering
	\includegraphics[width=0.95\textwidth]{figure/depth1111.pdf}
 	\vspace{-2mm}
	\caption{Qualitative results of different depth estimation methods. It shows that \textit{ToDER} yields an accurate depth estimation, especially the details indicated within the blue box.}
	\label{fig:depth_syn}
 	\vspace{-2mm}
\end{figure}

==> brief_sections/figures/pipeline1.tex <==
\begin{figure*}[ht]
	\centering
	\includegraphics[width=0.95\textwidth]{figure/pipeline333.pdf}
 	\vspace{0mm}
	\caption{Our depth estimation approach, To-and-fro Domain Adaptation for Colonoscopy Depth Estimation (ToDER), comprises a two-phase pipeline. In the initial phase, a CycleGAN is trained for domain adaptation between the source (Src) and target (Tgt) domains. Subsequently, the second phase involves co-supervising the source domain (Src) and the depth network (Depthnet) of the synthetic target domain using ground truth (GT) data from the source. Our method utilizes GANs for style transfer, employs TNet to refine depth results based on epipolar geometry constraints, and concludes with fine-tuning across all modules to enhance performance. Notably, our approach solely relies on depth information from the synthetic source domain, eliminating the need for target depth annotations.
 }
	\label{fig:pipeline1}
 	\vspace{-4mm}
\end{figure*}

==> brief_sections/figures/pipeline2.tex <==
\begin{figure*}[ht]
	\centering
	\includegraphics[width=0.8\textwidth]{figure/TMInewpipeline.pdf}
 	\vspace{0mm}
	\caption{The workflow of our method begins with an input colonoscopy video, which is initially segmented into individual RGB frames. Next, we apply our novel domain adaptation depth estimation technique, utilizing depth map data obtained from synthetic colonoscopy images. This enables the generation of depth maps for the actual colonoscopy RGB images. Subsequently, we employ Structure from Motion (SFM) to extract camera information and poses from the RGB images. Finally, we reconstruct the real colonoscopy scene by incorporating the depth maps along with their corresponding camera poses.
 }
	\label{fig:pipeline2}
 	 \vspace{-4mm}
\end{figure*}

==> brief_sections/figures/sythetic.tex <==
\begin{figure*}[ht]
	\centering
	\includegraphics[width=0.78\textwidth]{figure/syn2.pdf}
 	\vspace{-3mm}
	\caption{The reconstructed colons from synthetic data. The results are obtained through depth maps from the ground truth, our \textit{ToDER}, S2R-DepthNet, and Monodepth2. Compared to other approaches, our method showcases superior texture fidelity and continuity(red arrows), along with reduced noise levels(blue arrows).}
	\label{fig:synthetic}
 	\vspace{-4mm}
\end{figure*}

==> brief_sections/figures/sythetic2.tex <==
\begin{figure*}[ht]
	\centering
	\includegraphics[width=0.78\textwidth]{figure/Reconstruction.pdf}
 	\vspace{-3mm}
	\caption{The reconstructed colons used for quantitative evaluation. The results are obtained through depth maps from our \textit{ToDER}, S2R-DepthNet and Monodepth2.}
	\label{fig:synthetic2}
 	\vspace{-4mm}
\end{figure*}

==> brief_sections/figures/teaser.tex <==
\begin{figure}[!t]
	\centering
	\includegraphics[width=0.44\textwidth]{figure/recon_new.pdf}
 	\vspace{-3mm}
	\caption{Our reconstructed colon models from optical colonoscopy are displayed alongside comparisons on the right. We have employed MeshLab~\cite{cignoni2008meshlab} for visualizing our results, while the COLMAP~\cite{schonberger2016structure} outcomes are visualized using COLMAP itself. This choice enhances the clarity of COLMAP results, as their inaccurate reconstructions may obscure the accurate ones in MeshLab. The distinction of texture details and structure effectively underscores the superiority of our method.}
	\label{fig:real}
 	 \vspace{-4mm}
\end{figure}
